Shrouded Sin Taxes

Strategic shrouding of taxes by profit-maximizing firms can impair the effectiveness of corrective taxes. This paper explores tax shrouding and its consequences after the introduction of a digital sin tax designed to discourage harmful overconsumption of online sports betting in Germany. In response to the tax reform, most firms strategically shroud the tax, i.e., exclude tax surcharges from posted prices. Using an extensive novel panel data set on online betting odds, I causally estimate the effect of the tax on consumer betting prices. Consumers bear, on average, 76% of the tax burden. There is considerable and long-lasting heterogeneity in effects conditional on shrouding practices. Firms that shroud taxes can pass 90% of the tax onto consumers, while the pass-through rate is 16% for firms that directly post tax-inclusive prices. To understand the results' underlying mechanisms and policy implications, I propose an optimal corrective taxation model where oligopolistic firms compete on base prices and can shroud additive taxes. Tax shrouding is only attainable in equilibrium if (some) consumers underreact to shrouded attributes. According to the theoretical predictions, the empirically identified heterogeneity suggests that strategic tax shrouding significantly attenuates the positive corrective welfare effects of the tax. The results prompt regulating shrouding practices in the context of corrective taxation.

==> Chapters/Intro_digtax_diss.tex <==
Revenues in sports betting markets have experiences unprecedented growth over the past years \citep{montone2021optimal}. In Europe alone, \emph{online} gross betting revenues, i.e., the total wagered amount minus all winnings by bettors, grew from around \euro{}2.4bn in 2008 to over \euro{}12.1bn  in 2019 (H2 Gambling Capital 2021), making it "one of the fastest growing service activities in the EU" \citep{ec2012press}. Observers expect similar growth in North America after the US Surpreme Court overturned a law in 2018 that effectively banned commercial sports betting in most US states. 

One of the main arguments in favor of legalizing sports betting is that it provides a source of tax revenue to the government. Taxes on betting services is an classical example of a sin tax, that is usually levied on cigarettes, alcohl or or sugar drinks. 

Sin taxes are


In general, online betting services serve as a good example of a highly digitalized business model that poses several new regulatory and tax challenges to public authorities due to the lack of a required physical presence.\footnote{All three factors of highly digitalised business models, as defined by the \cite{oecd2014beps} apply to the online betting market: i) Cross-jurisdictional scale without mass, ii)  Reliance on intangible assets, including intellectual property (IP). iii)  Data, user participation and their synergies with IP.} Digitalization and deregulation transformed sports betting markets from segmented markets to a highly digitalized transnational market. This transformation


Against this background, this chapter examines the effect of the 2012 German (digital) sports betting tax on consumers' prices in online betting markets. The tax was introduced in July 2012 and imposed a 5\% duty on betting turnovers generated by German customers, which has to be paid by international betting agencies irrespective of their legal jurisdiction. I use a novel data set on betting odds from 68 international betting agencies for more than 80,000 sports events between 2009 and 2018, which allows me to infer implicit betting prices and estimate the tax effects over time. Considering that the average betting price on a single event, which is equal to the expected net return of a (random) bet from the perspective of a bookmaker, is only slightly higher than 7\% in the data set, the tax imposes a considerable levy on betting agencies.\footnote{Please note that overall gross betting margins of agencies tend to be higher, as many bettors "combine" bets, which means that all combined bets need to be successful. Combined bets multiplies the odds and thus the respective margins, which in turn increase the net return of the betting agencies per \$ wagered.}

To estimate the incidence of the tax over several years, I employ a difference-in-differences framework, comparing the change in betting prices of agencies that are active in the German market with changes in betting prices outside the German market. The estimated average pass-through on consumers is around 76\%. The incidence on consumers is very stable over time, and even shows a slightly increasing trend. 

I document three different endogenous "shrouding" policies of betting agencies in response to the new tax that affect the difference between the displayed, advertised tax-exclusive betting odds and the effective tax-inclusive betting odds. Contrary to predictions by the standard theory of tax incidence \citep{kotlikoff1987tax}, there is a large heterogeneity in the pass-through of the tax depending on the endogenous "shrouding" policies set by betting agencies. Agencies that choose to directly display the tax-inclusive odds are only able to shift a very small share of the betting tax onto consumers, roughly 16\% in the main specification. In contrast, agencies that advertise tax-exclusive odds, but deduct (the majority of) the tax after a specific bet is selected, either from potential winnings or the effective wager, are able to pass-through around 90\% of the tax onto consumer.\footnote{This result is confirmed by the assessment of one of the main competitors in their 2012 annual report, \cite{bwin2013annual}:  "Following the introduction of a 5\% turnover tax on sports betting in Germany on 1 July 2012, along with the rest of the industry, we began to pass on the majority of the tax to customers by requiring that winning customers pay a 5\% withholding on their pay-out".} This heterogeneity persist until the end of the observation period, even if the gap decreases over time. These considerable difference is not consistent with consumers that are perfectly informed and optimize fully with respect to tax-inclusive prices, assumed in the standard theory of taxation.\\
The tax salience literature, would argue that shrouding decreases the salience of taxes, which in turn increases the incidence on consumers because the tax elasticity is lower than the demand elasticity. Studies on tax salience \citep[e.g.][]{chetty2009salience, bradley2020hidden} usually assumes that the consumer pays the tax and that the salience of a tax is exogenously given. I extend the theoretical literature on tax salience, where the salience of the tax is dependent on "shrouding" policy by firms and where firms bear the statutory incidence of the tax. I propose a model populated with inattentive consumers and firms that can shroud taxes, combining insights from the tax salience literature \citep[e.g.][]{chetty2009salience} with studies on the shrouding of attributes and price obfuscation \citep[e.g.][]{gabaix2006}. The implications are...[That's were I am currently working at]   \\
Besides offering a promising natural experiment to study the heterogeneity of tax incidence when firms shroud taxes, the German sports betting tax also has important implications for the taxation in a digital world \citep[for a good overview of the challenges in digital taxation see:][]{oecd2014beps, devereux2020taxing} and the effect of sin taxes on online gambling and sports betting markets. Two topical aspects that can be expected to get increasingly relevant in the near future, given the very active discussion about the taxation of digital services and the rapid growth of the global market for online gambling in recent years. A trend that is expected to accelerate after the US Supreme court legalized sports betting in the US in 2018. [Add a number]. With respect to digital taxation, online betting services serve as a good example of a highly digitalized business model that poses several new regulatory and tax challenges to public authorities, common to many other newly digitalized markets.\footnote{All three factors of highly digitalised business models, as defined by the OECD (2019) apply to the online betting market: i) Cross-jurisdictional scale without mass, ii)  Reliance on intangible assets, including intellectual property (IP). iii)  Data, user participation and their synergies with IP.} \\
A first important insight of the study in the digital taxation context is that the international agencies seems to adhere to the German tax rules, despite a missing jurisdiction Germany. So, taxing digital services can work, in the sense, that they can generate considerable tax revenues even if the taxed entity has no jurisdiction within the respective country. Using data from a commercial provider that also serves the betting agencies and official bodies, I find that around 80\% and 90\% of sports betting revenue are taxed. In 2018, the total tax - paid by about 80 online betting agencies - was EUR 385m, which implies a total online betting revenue of EUR 7.7 billion in Germany, making it a significant source of tax revenue.\\
Concerning a potential corrective effect of betting taxes -- which is at the heart of the idea of sin taxes -- , my data is not granular enough to make a conclusive statement. However, overall betting revenues in Germany strongly increase and develop very similar to other European countries before and after the tax reform, which suggest a limited corrective effect of betting taxes. One of the likely sources of these limited effect are the salience effects and the respective "shrouding" policies by betting agencies. Forbidding such practices can be an effective tool to increase tax-exclusive prices and, in turn, the corrective effect of sin taxes on online betting consumption.\\
My study contributes to different strands of literature [to be added]\\
Behavioral public economics that report an increasingly number of anomalies, regarding tax incidence....
My findings are in line with a study by \cite{bradley2020hidden}, who find that introducing full-fare advertising rules, which required airlines and travel agents in the US to only advertise tax-inclusive prices on their website, lead to a sharp decreases (around 75\%) in the incidence of unit ticket taxes. This change is very similar to the estimated difference in pass-through of the online sports betting taxes conditional on different "shrouding policies", which provide some anecdotal evidence that the the level of sophistication, where consumers infer prices from the "shrouding" policy, appears rather low.\\
Add to the literature of "shrouding" by focusing on tax surcharges in a new market that is based in IO \\

The tax incidence is a central measure to evaluate the welfare and distributional effects of tax policies.\footnote{\cite{chetty2009salience} and \cite{weyl2013pass} show that tax incidence is often a sufficient statistics for various welfare analyses, both under perfect and imperfect competition.} The key results on tax incidence, such as tax neutrality, i.e., the economic incidence being independent of the statuary incidence, rest on the assumption that consumers are perfectly informed and optimize fully with respect to tax-inclusive prices. However, there is a very active literature that challenge these assumptions and results.\footnote{Examples include: \cite{sallee2011surprising}, \cite{goldin2013smoke}m \cite{Feldmann2015}, \cite{feldman2016}, \cite{kopczuk2016does}, \cite{benzarti2020goes} } In a seminal paper \cite{chetty2009salience} show that the behavioral responses to taxes strongly depend on the salience of the tax. One implication of their finding is that the tax incidence on consumers is lower when taxes are levied on producers "because producers must actively “shroud” a tax levied on them in order to reduce its salience". Consequently, the tax incidence should depend on how firms (can) shroud taxes, and forbidding the shrouding of taxes could be a cheap policy to decrease the incidence of taxes on consumers, which may be particularly relevant in the case of sin taxes.\footnote{\cite{bradley2020hidden} provide evidence on the effectiveness of such a policy in the context of US air carriers, finding a significant reductions in consumer tax incidence as a result of the policy that required online travel agents to incorporate all ticket taxes in advertised air ticket prices.} Following the arguments of \cite{gabaix2006}, it should further make a difference whether firms actively choose to shroud taxes or not if (a fraction of) consumers are sophisticated. Empirical evidence and theoretical implications on this channel are rare, as the tax salience literature usually assumes that tax salience is exogenous, independent of firms' strategic decisions and that the statutory incidence of a tax lies on consumers.\footnote{An emerging empirical literature on price partitioning highlights firms’ ability to increase consumer demand by not displaying the final price. In this respect a tax can be understood as a surcharge.  In particular, these studies demonstrate that when price components are shrouded or hidden such that the posted price is less than the all-inclusive price higher demand ensues. The lack of salience of the shrouded price components is the explanation typically put forth.} \\ 

==> Chapters/Literature.tex <==
\cite{montone2021optimal} did provide several descriptive results for the pricing in the global online betting market, using a cross-sectional data set on bookmakers' markup. He finds: i) the markup is inversely related to number of served marked segments and consumer quality; ii) positive association between the number of game outcomes and markup, potentially explained by an higher volatility of outcome or compensation of insider trading risks \citep[e.g.][]{shin1991optimal, shin1992prices, shin1993measuring}; iii) arbitrage opportunities exist



==> Chapters/Shrouding_price.tex <==
\subsection{"Shrouding" of tax surcharges and the difference between effective and posted betting prices}\label{sec:tax_shrouding}

On a website of a betting agency, the bettors can choose from numerous events in different leagues and for varying sports. Figure \ref{fig:odds_example} presents a typical example from a website of one of the main competitors.\footnote{The list on the left-hand side represents different leagues the bettor can choose from.} In the main panel of the example, you can find different events -- Premier Leaugue games in our example -- with respective odds for a Home win, Draw or Away win.\footnote{If you click on a particular game, there are also other betting types for the same game, such as the number of scored goals or spread bets.} Before bettors choose one particular bet, odds for different outcomes are always presented exclusive of a potential additional (tax) surcharge. While this surcharge directly relates to the sports betting tax and its magnitude (and framed in that way), there is, in principle, no direct link between the surcharge and the tax, as the tax has to be paid by suppliers, irrespective of agenices applying a surcharge or not. For this reason, I refer to the tax surcharge more generally to a surcharge, also to avoid confusion with net- and gross-betting prices in the theoretical analysis. Let denote the posted, advertised surcharge-exclusive odds as $\Tilde{r}_{isb}$.  

$\Tilde{r}_{isb}$ may differ from the effective surcharge-inclusive odds $r_{i,s,b}$, depending on endogenous "shrouding" policies set by the betting agencies. Accordingly, the surcharge-inclusive betting prices, $p_{ib}$,  may also differ from the implied advertised surcharge-exclusive betting prices $\Tilde{p}_{ib}$, which are equal to:
\begin{equation*}
   \Tilde{p}_{ib}=1- \dfrac{1}{\Tilde{\theta}_{ib}}
\end{equation*}
where $\Tilde{\theta}_{ib}=\sum_{s=1}^n \dfrac{1}{\Tilde{r}_{isb}}$ is the implied surcharge-exclusive markup for bookmaker $b$ and event $i$. Prior to the tax reform, there was no difference between advertised and effective betting prices, implying that $p_{ib}=\Tilde{p}_{ib}$. Let's denote $\tau$ as the difference between the effective and advertise betting prices:
\begin{equation*}
\tau=p_{ib}-\Tilde{p_{ib}}=\dfrac{1}{\Tilde{\theta}_{ib}}-\dfrac{1}{\theta_{ib}}
\end{equation*} 
If not stated otherwise, betting prices $p_{ib}$ always refer to the effective surcharge-inclusive betting prices.

As evident from some annual reports \citep[e.g.][]{bwin2013annual}, "shrouding" policies are an active decision by betting agencies to increase the effective betting prices after the introduction of the sports betting tax in Germany.\footnote{For instance, the 2012 annual report of "Bwin" makes the following statement: the "gross win margin [...] increased sharply in the second half [...] also because from August 2012 we began to withhold 5\% of players’ winning bets to cover the gaming tax due" \citep{bwin2013annual}.} There are, in principle, three different policies that betting agencies set that affect the difference between posted surcharge-exclusive and the effective surcharge-inclusive betting odds:\footnote{Betting agencies also use other ways to attract consumers that indirectly affect the effective (overall) betting prices, such as cash bonusses when a bettor deposits money on their account for the first time, loyalty bonusses that are usually "paid" out as free bets or trying to  "odds boost" that improve the effective odds if bettors combine a large number of bets. Historic data on these programs are not available. Using data from \textit{top100bookmaker} that provide a snapshot of bonus programs for several agencies in the year 2021, bonus programs seem not to vary considerably between betting agencies, so I abstract from differences in bonusses in this paper.}
\begin{itemize}
    \item[i)] \textbf{No further deductions}: The posted odds are equivalent to the effective odds: $r_{i,s,b}=\Tilde{r}_{isb}$. There is no difference between advertised and effective betting prices: $\tau=0$.
    \item[ii)] \textbf{Deducting tax surcharge from winnings}: In the case of a successful bet, the bettors receives only $(1-t)$ of the implied surcharge-exclusive payout. As a result, the effective tax-inclusive odds are equal to: $r_{i,s,b}=\Tilde{r}_{isb}(1-t)$. This implies: $\tau=\dfrac{t}{\Tilde{\theta}_{ib}}$.\footnote{See Appendix A on the derivation of $\tau$ for the different "shrouding" policies.}
    \item[iii)] \textbf{Deducting tax surcharge from wager}:  The tax surcharge applies directly to the effective wager, such that the effective wager multiplied by $(1+t)$ is equal to amount the bettor "bets"/pays. This implies that the effective tax-inclusive odds are equal to: $r_{i,s,b}=\dfrac{\Tilde{r}_{isb}}{(1+t)}$. This policy is a slightly more favorable to the bettor than policy ii), given that surcharge-exclusive odds equate (and $t>0$). In this case: $\tau=\dfrac{t}{(1+t)\Tilde{\theta}_{ib}}$.\footnote{Note that the idea behind this policy is that $t$ of the effective wager (after the tax surcharge is considered) is equal to the amount that is equal to }
\end{itemize}
In principle, betting agencies could also set policies in which the deductions are larger or smaller to $t$. Interestingly, there is no example of a betting agency that does that.\footnote{There is, however, one agency (Interwetten.com) that does not deduct the taxes if the bettor combines more than three games.} 

To get a better idea about the different shrouding policies turn again to the example above (Figure \ref{fig:odds_example}). Suppose a bettor wants to bet on a draw between Chelsea and Manchester City (marked by the red box). The posted tax-exclusive odds are equal to 3.30, implying that without further deduction the bettor, in case the game ends with a draw, would receive \euro{}3.30 for each \euro{}1 wagered . If the bettor choose one of the outcomes, draw in our example, there is a new panel popping up -- the betting slip ("Wettschein") -- that has an input window for the amount a bettor wants to wager. After the amount is entered the potential net payout, tax-inclusive odds multiplied by the wager, are calculated and presented to the bettor. This is the first time during the interaction with the website where tax-inclusive odds can be directly inferred by the bettor.

Figure \ref{fig:policies} illustrates examples of such a betting slip of three different betting agencies that use different "shrouding" policies for the same bet (Draw in the game Chelsea vs. Manchester City). Panel ii) refers to the betting agency in our example in Figure \ref{fig:odds_example} that use "shrouding" policy ii): "Deducting tax from winnings". As you can see in Figure \ref{fig:policies} Panel ii), a bet of \euro{}100 would not result in a potential net payout of \euro{}330 as implied by the tax-exclusive odds of 3.30 but only in \euro{}313.50, which is equal to $330*(1-0.05)$.\footnote{The yellow button "Einzahlen" button translates to Deposit, as the bettor has no money in her account. If the bettor has sufficient funds, the yellow button would place the bet.} In contrast, the betting agency in panel i) does not impose further deductions on the posted odd, implying that the potential net payout is equal to the wager times the posted odds, \euro{}330 in our example. To advertise that there are no further tax surcharges ("Gebühr") on this website, the bookmaker additionally displays the surcharges a bettor would pay with a bookmaker that deducts 5\% of the winnings as in the previous example (\euro{}16.50), see the crossed-out red number. Panel iii) illustrates an example of an agency that employs the third policy deducting a surcharge from the effective wager.\footnote{Please note that the bookmaker in this example uses $t=0.053$, the new tax rate after the reform in July 2021. Before the reform, the agency used $t=0.05$ as well.} The tax-exclusive odds for this agency is only equal to 3.15. Compared to the agency in Panel ii), the agency is more transparent how the net payout ("Möglicher Gewinn") is calculated, displaying the steps of the underlying calculation, including effective wager ("Effektiver Einsatz") and the "tax" ("Steuer") directly.\footnote{The presentation of the betting slip for other agencies by "shrouding" policies looks very similar, see Appendix.} In general, it is noteworthy that the agency always refer to the surcharge as "tax", similar to a VAT, which gives the impression that the agencies are bound to pass the tax onto consumers.


==> Chapters/Theory_simple.tex <==


\section{A consumer search model of tax shrouding}

Suppose a unit mass of firms $k \in [0,1]$ supply a differentiated product $x_k$ at zero marginal costs. Selling the product is subject to an excise tax $t$ that has to be remitted by the firms. Firms set a salient posted price $p^s_k$ and a shrouded tax surcharge $\tau_k$, which can be either zero or equal to the unit tax $t$ ($\tau_k \in \{0, t\}$). Unshrouding of the tax surcharge ($\tau_k=0$) comes at cost $0\leq \psi<t$ per product. Accordingly, the firm $k$'s consumer price is defined as $p_k=p^s_k+\tau_k$ and producers prices are $p_k-t$.

There is a unit mass of consumers $i \in  [0,1]$ that seek to purchase at most one product and spend their remaining budget $W$ on an untaxed numeraire good $z$ that is supplied in a perfectly competitive market. Assume for now that the utility is linear in $z$. Consumer $i$ values the good with $\omega_{ik}>0$. $\omega_{ik}$ is a exogenous firm-consumer specific match value representing idiosyncratic product fit that is independently distributed according to distribution function $F$ and density function $f$ on the support $[\Bar{\omega}, \underline{\omega}]$. %\footnote{I make this assumption for a better tractability of the model. Qualitatively similar results would emerge if we make the less restrictive assumption of an increasising hazard rate property, i.e. $1-F(.)$ is log-concave \citep{anderson2018firm}} 
Let %$U_{i}=u(z)+v_{ik}$ denote the true utility of consumer $i$ (net of any search costs) where 
$v_{ik}$ denote individual $i$'s true utility from purchasing good $k$:
\begin{equation*}
    v_{ik}= \mu\omega_{ik}-(p^s_k+\tau_k)=\mu\omega_{ik}-p_k,
\end{equation*}
where $\mu$ is scaling parameter reflecting the degree of taste and product heterogeneity ($\mu=0$ implies an homogeneous product). For now suppose that $\mu=1$ 

Consumers search one product at a time in a random order and with perfect recall. Visiting a firm entails search costs $s>0$ and there is no upper limit in the number of firms searched. There are two types of consumers. A fraction $\lambda \in [ 0,1 ]$ of consumers is sophisticated and learn $p_k$, $\tau_k$ and the firm-consumer specific match value $\omega_{ik}$ upon visiting firm $k$. The remaining $1-\lambda$ consumers are naive and misperceive the shrouded tax surcharge being equal to $\theta t$ if $\tau_k=t$. $\theta$ can be interpreted as a tax salience parameter similar to \citet{chetty2009salience, dellavigna2009psychology}. Naive consumer further do not observe their product fit and act as if all the products provide average fit $\Tilde{\omega}$.

%They are randomly assigned to one firm and hold the belief that unobserved tax surcharge is zero. Consequently, the naive consumers buy from the randomly assigned firm if and only if $u(Z-p_k)+\omega_{ik}\geq u(Z)$.\footnote{The results would qualitatively not change if we allow the naive consumers to search as well.}

The timeline of the model is as follows: i) firms simultaneously and non-cooperatively set their strategy profile, consisting of $p^s_k$ and $\tau_k$; ii) consumers make their search and purchase decision. It is well-know that in these type of search models, following \citet{wolinsky1986true} and \citet{anderson1999pricing}, . Thus, the consumers' strategy is a search rule that specifies whether to end search or end search conditional on past search history. 
Denote $\Tilde{u}$ as the utility that the consumer would receive if she choose to not buy the product. Suppose the consumer searches, alternative one with (perceived) utility $v^p_{i1}$ will be purchased if $v^p_{i1}>\Tilde{u}$ (implying that the consumer does not search when she is indifferent). Otherwise the consumer chooses the outside option. It is therefore optimal to search if and only if:

\begin{equation}
    E(\max\{v^p_{i1}-\Tilde{u},0\}=\int^{\infty}_{\Tilde{u}} {(x-\Tilde{u})dG(x)}>s
\end{equation}




If $s$ tends to zero, we have marginal cost pricing $p^*=t$. We assume that s is small enough, such that consumer does not gives up searching.

When 


\subsubsection*{Benchmark with only sophisticated consumers}

As a baseline we consider a market that is only populated by sophisticated consumers. For sophisticated consumers, tax and price elasticities equate. Accordingly, the maximization problem of the firms can be written in terms of the effective consumer prices $p_k$. In the derivation of the demand for sophisticated consumers we follow \citet{wolinsky1986true} and \citet{anderson1999pricing} considering only equlibria where all firms choose the same price $p^*$. Thus, a sophistcated consumer assumes that all not-visited firms charge $p_k=p^*$, which holds true even if consumers observe a deviation from the equilibrium price in the first search. 


Suppose the first firm $j$ has set price $p_j$ (allowing for off-equilibrium pricing). If Thus, the associated individual utility is equal to $v_{ij}= \omega_{ij}-p_j$. If the consumer visits another firm $l$ she will prefer to buy the new product if $\omega_{ij}-p_j+p^*>\omega_{il}$. The expected incremental utility from searching one firm more is given by:


I follow \citet{anderson2001tax} and consider symmetric differentiated demand systems in which demand for firm $i$’s product can be written as $D(p_k, p_{-k})$ that is assumed to be continuously differentiable. The demand for product $k$ is decreasing in $p_k$ and increasing in $p_{-k}$, the common price charged by other firms. Firm $i$'s profit can be written as:
\begin{equation*}
    \pi_{k}= (p_k-t)D(p_k, p_{-k})
\end{equation*}

\begin{equation*}
    D(p_k, p_{-k})=1-F(\hat{\theta}
\end{equation*}

The strategic interaction between firms is described by a Bertrand-Nash game. The first-order condition defines the firms' best replies conditional on all other firms choose common price $p_{-k}$:

\begin{equation*}
    (p_k-t)\dfrac{\delta D(p_k, p_{-k})}{\delta p_k} + D(p_k, p_{-k})=0
\end{equation*}

\subsubsection*{Benchmark with only naive consumers}




%Suppose all consumers observe the posted price but only a fraction $\lambda$ of consumers observe each firm's tax surcharge.  A fully optimizing consumer purchases the good ($x=1$) if and only if $u(Z-p_k)+_i\geq u(Z)$


%Do I need a match value between consumer and firm



The effective total price of $x$ is $p=p_s+\tau$, which can be decomposed in a salient posted price $p_s$ and a shrouded tax surcharge set by firms $\tau$.  . A fully optimizing consumer purchases the good ($x=1$) if and only if $u(Z-p_k)+v_{ik}\geq u(Z)$.



\footnote{The utility is sucht that it does not depend on the past consumption of the sin good \citep{gruber2004tax}}

In the absence of the tax, both type of consumers optimize perfectly. $x_i*(p, t, Z)$

% There are two types of consumers: i) myopic consumers who decide only based on the displayed price. They are completely inattentive to the tax surcharges ($\psi=0$); ii) sophisticated consumers always take taxes into account. 

% when  Timeline:

% \begin{itemize}
%     \item[1.] Firms set displayed prices decide whether to pass on taxes or not. In the base case, firms can only shroud the entire tax or nothing.
%     \item[2.] Consumers choose a firm based on the expectation about post tax prices. The prior belief about post reform prices refer to historical pre-tax prices. Sophisticated consumers (Share: $0\leq \alpha \leq 1$) observe the tax decision and take them into account as a signal whether it is high or low price firm. Myopic consumers (Share: $0\leq 1-\alpha \leq 1$) choose a firm based on prior beliefs.
%     \item[3.] Consumers choose how much they want to bet. Sophisticated consumers optimize their consumption based on tax-inclusive prices independent decision ($p=q+t$). Myopic consumers choose based on the displayed prices only. 
% \end{itemize}

% Tradeoff of firms: i) no tax surcharge, implying lower effective prices/margins plus more demand from and share of sophisticated consumers that choose their website; ii) set tax surcharge: Tax is completely passed on to myopic consumers without negative effects from them, lower demand from and less sophisticated consumers



==> Chapters_rel_pricing/Intro_rel.tex <==
Wagering markets have long-standing tradition of being a natural asset pricing laboratory to test market efficiency and rationality. Two key features allows a direct test of mispricing in betting markets that circumvent the joint hypotheses problem \citep{fama1970efficient}: i) wagering markets have have a well-defined termination point at which its value become certain \citep[e.g.][]{thaler1988anomalies}; ii) sport bets are idiosyncratic and independent of systematic risk in an economy \citep{moskowitz2021asset}. The effects of financial transaction taxes on market efficiency is very complex and empirical evidence is very rare.   

The effect of financial transaction taxes on market efficiency is no in general really complex 

Wagering markets have a well-defined termination point at which its value become certain, which make them better suited to test market efficiency and rationality \citep{thaler1988anomalies}.

==> Chapters_rel_pricing/literature_rel.tex <==
\cite{sauer2005state} provides a discussion of the early literature on wagering markets that mainly focused on testing the efficient markets hypothesis. He calls for more in innovative approaches to exploit the "rich source of knowledge on the process of price
formation and the information content of market prices". He concludes "are packed with information that is worth extracting." 


There is a vast literature that uses data on betting markets to test the efficient market hypothesis: \cite{snyder1978horse, figlewski1979subjective, hausch1981efficiency, asch1982racetrack} horse racetrack betting  \cite{pankoff1968markets, zuber1985beating, gandar1988testing, golec1991degree, zuber1985beating, gray1997testing} use point spreads data on American Football games; \cite{woodland1994market} on baseball games: on Basketball games \cite{camerer1989does} Basket ball games. All of these studies use data of a single bookmaker


vast  paper use data on various betting markets to test the efficient market hypothesis. In these studies, "efficiency implies that odds or prices summarize all that is known about an event, and more generally, the absence of profitable betting opportunities." \cite{sauer2005state}. The evidence on the efficiency is mixed. Early studies find that the efficiency hypothesis cannot be rejected \citep[e.g.][]{pankoff1968market, sauer1988hold, }. Odds at the racetrack  \citep{}. To the contrary, there are, however, several studies that reject efficient pricing. Several biases that may serve as an explanation have been identified:

\begin{itemize}
    \item Horse racing Favorite longshot bias: \cite{asch1982racetrack}
    \item NFL: Bias against home teams, bias against underdogs \citep{golec1991degree}
    \item UK football betting: Same favorite longshot bias as in horse racing
    \item The favorite longshot bias  , the reverse is shown for baseball markets \cite{woodland1994market}
    \item The "hot hand fallacy" where players continue to hit \citep{camerer1989does}
    \item the underbetting of home underdogs in American Football \citep{paul2003fair}
\end{itemize}

Potential reasons of "mispricing": misperception of bettors \citep[e.g. the hot hand ][]{}

Pricing of book makers:

There are several studies that look into markoff of single bookmakers, usually assuming a constant markup \citep{levitt2004gambling}

\cite{dare1996generalized} provide a generalized model to test market efficiency and rationality, taking into account the interdependencies between playing at home (away) and being the favorite (the underdog). Their approach apllies to point spread markets.

"The defining characteristic of rational expectations requires market probability
distributions of economic variables, conditional on available information, to be
equal to objective probability distributions, conditional upon the same informa-
tion set" \cite{gandar1988testing}

Results are mixed: certain studies
have found these markets to be efficient (Snyder 1978; Ali 1979;
Figlewski 1979); others have found inefficiencies that allow for
profitable wagering (Hausch, Ziemba, and Rubinstein 1981; Asch,
Malkiel, and Quandt 1984).

==> Chapters_rel_pricing/theory_ratios.tex <==

\subsection{The price of a bet}

Bets have a direct application to financial markets as they constitute simple state-contingent claims and can be understood as an Arrow-Debreu (pure state) securities. The payoffs are linearly independent, the payoff matrix has a full rank (complete markets) and each state can be "insured" individually. Bets have a well-defined expiration date, the end of an specific event, when its value becomes certain. The inverse of $q_{i, s,b}$ can be directly translated into a state price that pays the bettor 1\$ if state s is realized. Take a football match between Team 1 and Team 2 as an example. There are three potential (future) states of the world ($n=3$): Team 1 wins; Draw; Team 2 wins). A \$1 bet on Team 1 can be represented by following payout vector: $(\$q_1, 0, 0)$, a bet on a draw: $(0,\$q_2,0)$ a bet one Team 2: $(0, 0, \$q_3)$. If we abstract from potential limits to the wagered amount, all systems of "markets" in betting are complete  as we can spans the space of all conceivable payoff vectors given our states of the world with no redundant bet.\footnote{We abstract from a dynamic component and set the risk free rate equal to one.}

Accordingly, the markup of betting agency $b$ for state $s$ is equal to the ratio between the implied probability(state price $\Tilde{\pi}=\dfrac{1}{q_{i,s,b}}$ and the unobserved true probability:
\begin{equation}
\label{eqn:singlemargin}
    \theta_{i, b}=\dfrac{\Tilde{\pi}_{i, s}}{\pi_{i, s}},
\end{equation}

Expected rate of return of 1\$ bet on outcome $i$:

\begin{equation}
   E_i=\pi_i(q_i-1)-(1-\pi_i)=1/\theta_{i, b}-1
\end{equation}


There are $n$ mutually-exclusive states of the world ($s=1,2,...n$) defined by the outcomes of a particular event $i$. Bookmaker $b$ promises bettors to pay odd $q_{i, s,b}$ for every \$1 wagered if state $s$ is realized and zero otherwise.\footnote{I use the decimal odds notation in this paper that directly refers to this definition. The two other common notations are fractional (or English) odds and moneyline (or American) odds. The odds can be converted as follows:}  The odd for an arbitrary state $s$ for a specific event $i$ can be expressed as:
\begin{equation}
\label{eqn:singlemargin}
    q_{s,b}=\dfrac{1}{\theta_{s, b} \pi_{s}},
\end{equation}
where $\pi_{i, s}$ represents the (objective) likelihood of state $s$. $\theta_{s, b}$ is bookmaker $b$'s markup (for event $i$) and state $s$. Accordingly, the markup is not fixed and can vary across different events and conditional on characteristics of the state, such as the objective likelihood or home or away win. 

Bets have a direct application to financial markets as they constitute simple state-contingent claims and can be understood as an Arrow-Debreu (pure state) securities. The payoffs are linearly independent, the payoff matrix has a full rank (complete markets) and each state can be "insured" individually. Bets have a well-defined expiration date, the end of an specific event, when its value becomes certain. Take a football match between Team 1 and Team 2 as an example. 
For now we focus on the investment decision of one bettor and the pricing decision of one bookmaker for a particular event. There are three potential (future) states of the world ($n=3$): Team 1 wins; Draw; Team 2 wins). A \$1 bet on Team 1 can be represented by following payout vector: $(\$q_1, 0, 0)$, a bet on a draw: $(0,\$q_2,0)$ a bet one Team 2: $(0, 0, \$q_3)$. If we abstract from potential limits to the wagered amount, all systems of "markets" in betting are complete  as we can spans the space of all conceivable payoff vectors given our states of the world with no redundant bet.\footnote{We abstract from a dynamic component and set the risk free rate equal to one.}
There are two dates: today (t=0) and end of the match (t=1)
The expected profit of a single bookmaker in one event is given by:

\begin{equation*}
    E_0(Pr)=\sum_s \pi_s(1-q_s E(\psi_s))=1-\sum_s (\dfrac{1}{\theta_{s}} E(\psi_s))=,
\end{equation*}

where $\psi_s$ is equal to the overall share of bettors that bet on event $s$. If beliefs are unbiased.


\subsubsection{Consumers}

We consider a single Arrow Debreu problem. Consumers are endowed with wealth $W$ and take prices as given. $c_0$ represent consumption in period $0$ and $c_s$ consumption in state $s$, which depends on the realization of the event. I abstract from a time discount factor here. Consumers maximize following problem: 

\begin{equation*}
    \max v(c_0) + \sum_s E(\pi_s) u(c_s)
\end{equation*}
s.t. 
\begin{equation*}
    c_0 + \sum_s q_s c_s = W
\end{equation*}
The first order conditions of the corresponding Lagrangian are equal to:

\begin{equation*}
    v'(c_0)=\lambda
\end{equation*}

\begin{equation*}
    u'(c_s)=\lambda \dfrac{q_s}{E(\pi_s)},
\end{equation*}

which implies that 

\begin{equation*}
    \dfrac{u'(c_s)}{u'(c_s')}= \dfrac{\dfrac{q_s}{E(\pi_s)}}{\dfrac{q_s'}{E(\pi_s')}} = \dfrac{\theta_s}{\theta_{s'}} ,
\end{equation*}


\begin{equation*}
    max E_0(Pr)=1-\sum_s (\dfrac{1}{\theta_{s}} E(\psi_s))=,
\end{equation*}


Consumer optimality condition implies that ratio of marginal utilities is equal across states

is equal to:

\begin{equation*}
    \dfrac{\Tilde{\pi}_s U'(c_s)}{\Tilde{\pi}_{\Bar{s}} U'(c_{\Bar{s}})}=\dfrac{q_{\Bar{s}}}{q_s}
\end{equation*}

\subsubsection{Agencies}

Are agencies able to exploit misperceptions by bettors?

==> Diff_in_Diff_Soccer.tex <==
\begin{table}[htbp]\centering
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\caption{Panel B: Soccer - all agencies}
\scalebox{0.6}{
\begin{tabular}{l*{8}{c}}
\hline\hline

                    &\multicolumn{4}{c}{All Leagues}     &\multicolumn{4}{c}{Excl. "cross" leagues}     \\
                    
                    &\multicolumn{1}{c}{(1)}      &\multicolumn{1}{c}{(2)}      &\multicolumn{1}{c}{(3)}      &\multicolumn{1}{c}{(4)}      &\multicolumn{1}{c}{(5)}      &\multicolumn{1}{c}{(6)}      &\multicolumn{1}{c}{(7)}      &\multicolumn{1}{c}{(8)}      \\

\hline
treated             &               0.048\sym{***}&               0.048\sym{***}&               0.049\sym{***}&               0.049\sym{***}&               0.053\sym{***}&               0.053\sym{***}&               0.054\sym{***}&               0.054\sym{***}\\
                    &             (0.006)         &             (0.004)         &             (0.004)         &             (0.004)         &             (0.006)         &             (0.003)         &             (0.003)         &             (0.003)         \\
[0.2em]
tax\_dummy           &              -0.020\sym{***}&              -0.016\sym{***}&                             &                             &              -0.020\sym{***}&              -0.017\sym{***}&                             &                             \\
                    &             (0.003)         &             (0.003)         &                             &                             &             (0.003)         &             (0.003)         &                             &                             \\
[0.2em]
GER\_dummy           &               0.000         &                             &                             &                             &               0.004         &                             &                             &                             \\
                    &             (0.006)         &                             &                             &                             &             (0.005)         &                             &                             &                             \\
[0.2em]
Constant            &               0.090\sym{***}&               0.079\sym{***}&               0.085\sym{***}&               0.093\sym{***}&               0.089\sym{***}&               0.078\sym{***}&               0.085\sym{***}&               0.100\sym{***}\\
                    &             (0.004)         &             (0.002)         &             (0.003)         &             (0.003)         &             (0.004)         &             (0.002)         &             (0.004)         &             (0.004)         \\
\hline
Agency fixed effects&                  No         &                 Yes         &                 Yes         &                 Yes         &                  No         &                 Yes         &                 Yes         &                 Yes         \\

Time fixed effects  &                  No         &                  No         &                 Yes         &                 Yes         &                  No         &                  No         &                 Yes         &                 Yes         \\

League fixed effects&                  No         &                  No         &                  No         &                 Yes         &                  No         &                  No         &                  No         &                 Yes         \\
\hline
Observations        &             1852271         &             1852271         &             1852271         &             1852271         &             1247260         &             1247260         &             1247260         &             1247260         \\
\(R^{2}\)           &               0.231         &               0.608         &               0.633         &               0.768         &               0.166         &               0.587         &               0.620         &               0.750         \\
\hline\hline
\multicolumn{9}{l}{\footnotesize Standard errors in parentheses}\\
\multicolumn{9}{l}{\footnotesize \sym{*} \(p<0.05\), \sym{**} \(p<0.01\), \sym{***} \(p<0.001\)}\\
\end{tabular}
}
\end{table}


==> Diff_pres_het.tex <==
\begin{table}[ !ht]\centering
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\caption{Effects of tax on consumer betting prices are heterogeneous}
    \label{diffindiff_het}
\scalebox{0.55}{
\begin{tabular}{l*{7}{c}}
\hline\hline

                 &\multicolumn{3}{c}{All Leagues}     & &\multicolumn{3}{c}{Excl. "cross" leagues}     \\    \cmidrule{2-4} \cmidrule{6-8}
                                  &\multicolumn{2}{c}{Subsamples}     & Interact. & &\multicolumn{2}{c}{Subsamples} &  Interact.  \\    \cmidrule{2-3} \cmidrule{6-7}
                    &\multicolumn{1}{c}{No shrouding}      &\multicolumn{1}{c}{Shrouding}      &   &   &\multicolumn{1}{c}{No shrouding}      &\multicolumn{1}{c}{Shrouding}      &   \\
                    &\multicolumn{1}{c}{(1)}      &\multicolumn{1}{c}{(2)}      &\multicolumn{1}{c}{(3)}   &   &\multicolumn{1}{c}{(4)}      &\multicolumn{1}{c}{(5)}      &\multicolumn{1}{c}{(6)}      \\
\midrule

Tax effect on prices             &               0.008\sym{***}&               0.041\sym{***}&                             &   &            0.008\sym{**} &               0.045\sym{***}&                             \\
                 &             (0.002)         &             (0.003)         &                             &   &          (0.002)         &             (0.003)         &                             \\
[1em]
$T_{i,m}$           &                             &                             &               0.046\sym{***}&   &                          &                             &               0.050\sym{***}\\
                    &                             &                             &             (0.003)         &  &                           &                             &             (0.003)         \\
[1em]
$T_{i,m}$ x $no Shroud_{i,m}$            &                             &                             &              -0.041\sym{***}&  &                           &                             &              -0.043\sym{***}\\
                    &                             &                             &             (0.002)         &  &                           &                             &             (0.002)         \\
[1em]
Constant            &               0.085\sym{***}&               0.084\sym{***}&               0.084\sym{***}& &              0.091\sym{***}&               0.091\sym{***}&               0.091\sym{***}\\
                    &             (0.003)         &             (0.003)         &             (0.003)         & &            (0.003)         &             (0.003)         &             (0.003)         \\
\midrule
Time FE             &                 Yes         &                 Yes         &                 Yes         &  &               Yes         &                 Yes         &                 Yes         \\
Agency FE           &                 Yes         &                 Yes         &                 Yes         &  &               Yes         &                 Yes         &                 Yes         \\
League FE           &                 Yes         &                 Yes         &                 Yes         &   &              Yes         &                 Yes         &                 Yes         \\
\hline
Observations        &             1,587,090         &             1,881,406         &             1,936,322         &   &          1,211,548         &             1,277,394         &             1,290,843         \\
\(R^{2}\)           &               0.728         &               0.767         &               0.779         &  &             0.737         &               0.757         &               0.761         \\
\hline\hline
\multicolumn{7}{l}{\footnotesize Standard errors in parentheses. \sym{*} \(p<0.05\), \sym{**} \(p<0.01\), \sym{***} \(p<0.001\)}\\
\end{tabular}
 }
\end{table}

==> Diff_pres_het2.tex <==
\begin{table}[ !ht]\centering
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\caption{Effects of tax on consumer betting prices are heterogeneous}
    \label{diffindiff_het}
\scalebox{0.65}{
\begin{tabular}{l*{4}{c}}
\hline\hline


                                  &\multicolumn{2}{c}{Subsamples}     & Interact. \\    \cmidrule{2-3}
                    &\multicolumn{1}{c}{No shrouding}      &\multicolumn{1}{c}{Shrouding}      &   \\
                    &\multicolumn{1}{c}{(1)}      &\multicolumn{1}{c}{(2)}      &\multicolumn{1}{c}{(3)}     \\
\midrule

Tax effect on prices             &               0.008\sym{***}&               0.041\sym{***}&                             \\
                 &             (0.002)         &             (0.003)         &                            \\
[1em]
$T_{i,m}$           &                             &                             &               0.046\sym{***}\\
                    &                             &                             &             (0.003)          \\
[1em]
$T_{i,m}$ x $no Shroud_{i,m}$            &                             &                             &              -0.041\sym{***}\\
                    &                             &                             &             (0.002)         \\

\midrule
Constant         &                 Yes         &                 Yes         &                 Yes        \\
Time FE             &                 Yes         &                 Yes         &                 Yes        \\
Agency FE           &                 Yes         &                 Yes         &                 Yes      \\
League FE           &                 Yes         &                 Yes         &                 Yes         \\
\hline
Observations        &             1,587,090         &             1,881,406         &             1,936,322             \\
\(R^{2}\)           &               0.728         &               0.767         &               0.779              \\
\hline\hline
\multicolumn{4}{l}{\footnotesize Standard errors in parentheses. \sym{*} \(p<0.05\), \sym{**} \(p<0.01\), \sym{***} \(p<0.001\)}\\
\end{tabular}
 }
\end{table}

==> Diff_pres_het_pol.tex <==
\begin{table}[ !ht]\centering
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\caption{Avg. effect of tax on consumer betting prices - Subsamples different policies}
    \label{diffindiff_het_pol}
\scalebox{0.45}{
\begin{tabular}{l*{7}{c}}
\hline\hline

                 &\multicolumn{3}{c}{All Leagues}     & &\multicolumn{3}{c}{Excl. "cross" leagues}     \\    \cmidrule{2-4} \cmidrule{6-8}
                 
 "Shrouding" policy                   &\multicolumn{1}{c}{(ii)}      &\multicolumn{1}{c}{(iii)}      &\multicolumn{1}{c}{(i)}   &   &\multicolumn{1}{c}{(ii)}      &\multicolumn{1}{c}{(iii)}      &\multicolumn{1}{c}{(i)}      \\
 [0.3em]
                     &\multicolumn{1}{c}{(1)}      &\multicolumn{1}{c}{(2)}      &\multicolumn{1}{c}{(3)}   &   &\multicolumn{1}{c}{(4)}      &\multicolumn{1}{c}{(5)}      &\multicolumn{1}{c}{(6)}      \\
                    

\midrule
\textbf{Panel A: Soccer} &&&&&&& \\
[1em]
Tax effect on prices              &               0.043\sym{***}&               0.036\sym{***}&               0.008\sym{***}& &              0.046\sym{***}&               0.043\sym{***}&               0.008\sym{**} \\
                    &             (0.003)         &             (0.007)         &             (0.002)         &  &           (0.003)         &             (0.005)         &             (0.002)         \\
[1em]
Constant            &               0.085\sym{***}&               0.085\sym{***}&               0.085\sym{***}&       &        0.091\sym{***}&               0.091\sym{***}&               0.091\sym{***}\\
                    &             (0.003)         &             (0.003)         &             (0.003)         &   &          (0.003)         &             (0.003)         &             (0.003)         \\

\hline
Observations        &             1,793,974         &             1,619,606         &             1,587,090         &   &          1,257,582         &             1,217,911         &             1,211,548         \\
\(R^{2}\)           &               0.764         &               0.743         &               0.728         &   &            0.754         &               0.743         &               0.737         \\

\midrule
\textbf{Panel B: All sports} &&&&&&& \\
[1em]
Tax effect on prices             &               0.044\sym{***}&               0.034\sym{***}&               0.002     &    &               0.041\sym{***}&               0.037\sym{***}&               0.001         \\
                    &             (0.002)         &             (0.007)         &             (0.002)         &   &          (0.002)         &             (0.007)         &             (0.002)         \\
[1em]
Constant            &               0.079\sym{***}&               0.084\sym{***}&               0.084\sym{***}&   &            0.088\sym{***}&               0.088\sym{***}&               0.088\sym{***}\\
                    &             (0.003)         &             (0.003)         &             (0.003)      &   &             (0.003)         &             (0.003)         &             (0.003)         \\

\midrule
Observations        &             2,815,902         &             2,512,623         &             2,466,796         &    &         1,974,102         &             1,912,848         &             1,901,791         \\
\(R^{2}\)           &               0.745         &               0.716         &               0.703         &    &           0.736         &               0.721         &               0.713         \\
\midrule
Time FE             &                 Yes         &                 Yes         &                 Yes         &         &        Yes         &                 Yes         &                 Yes         \\
Agency FE           &                 Yes         &                 Yes         &                 Yes         &      &           Yes         &                 Yes         &                 Yes         \\
League FE           &                 Yes         &                 Yes         &                 Yes         &   &              Yes         &                 Yes         &                 Yes         \\
\hline\hline
\multicolumn{7}{l}{\footnotesize Standard errors in parentheses}\\
\multicolumn{7}{l}{\footnotesize \sym{*} \(p<0.05\), \sym{**} \(p<0.01\), \sym{***} \(p<0.001\)}\\
\end{tabular}
}
\end{table}


==> DiffinDiff_Table.tex <==

\begin{table}[ !ht]\centering
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\caption{Bettors bear most of the effective tax burden}
\label{diffindiff_soccer}
\scalebox{0.6}{
\begin{tabular}{l*{7}{c}}
\hline\hline

                 &\multicolumn{3}{c}{All Leagues}     & &\multicolumn{3}{c}{Excl. "cross" leagues}     \\    \cmidrule{2-4} \cmidrule{6-8}
                    &\multicolumn{1}{c}{(1)}      &\multicolumn{1}{c}{(2)}      &\multicolumn{1}{c}{(3)}   &   &\multicolumn{1}{c}{(4)}      &\multicolumn{1}{c}{(5)}      &\multicolumn{1}{c}{(6)}      \\

\midrule

\textbf{Panel A: All agencies} &&&&&&& \\
[1em]
Tax effect on prices             &               0.038\sym{***}&               0.038\sym{***}&               0.038\sym{***}&   &            0.041\sym{***}&               0.041\sym{***}&               0.041\sym{***}\\
                    &             (0.004)         &             (0.004)         &             (0.004)       &  &             (0.005)         &             (0.005)         &             (0.005)         \\

\hline
Observations        &             1,936,322         &             1,936,322         &             1,936,322       &  &             1,290,843         &             1,290,843         &             1,290,843         \\
\(R^{2}\)           &               0.642         &               0.759         &               0.811      &   &               0.643         &               0.754         &               0.809         \\
\midrule
\textbf{Panel B: Completed agencies} &&&&&&& \\
[1em]
Tax effect on prices           &               0.038\sym{***}&               0.038\sym{***}&               0.038\sym{***}&  &             0.041\sym{***}&               0.041\sym{***}&               0.041\sym{***}\\
                    &             (0.005)         &             (0.005)         &             (0.005)      &   &             (0.005)         &             (0.005)         &             (0.005)         \\


\hline
Observations        &             1,276,400         &             1,276,400         &             1,276,400         &    &          778,207         &              778,207         &              778,207         \\
\(R^{2}\)           &               0.521         &               0.699         &               0.747         &   &            0.467         &               0.660         &               0.711         \\

\midrule

Constant            &                 Yes         &                 Yes         &                 Yes       &  &                 Yes         &                 Yes         &                 Yes         \\

Time FE             &                 Yes         &                 Yes         &                 Yes    &     &                 Yes         &                 Yes         &                 Yes         \\

Agency FE           &                 Yes         &                 Yes         &                  No       &  &                 Yes         &                 Yes         &                  No         \\

League FE           &                  No         &                 Yes         &                  No     &    &                  No         &                 Yes         &                  No         \\

League-agency FE    &                  No         &                  No         &                 Yes      &   &                  No         &                  No         &                 Yes         \\
\hline \hline
\multicolumn{7}{l}{\footnotesize Standard errors in parentheses. \sym{*} \(p<0.05\), \sym{**} \(p<0.01\), \sym{***} \(p<0.001\)}\\
\end{tabular}
}
\end{table}



==> DiffinDiff_Tablepres.tex <==

\begin{table}[ !ht]\centering
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\caption{Bettors bear most of the effective tax burden}
\label{diffindiff_soccer}
\scalebox{0.62}{
\begin{tabular}{l*{8}{c}}
\hline\hline

                 &\multicolumn{2}{c}{All Leagues}     & &\multicolumn{2}{c}{Excl. "cross" leagues} & & \multicolumn{2}{c}{Compl. agencies}    \\    \cmidrule{2-3} \cmidrule{5-6} \cmidrule{8-9}
                    &\multicolumn{1}{c}{(1)}      &\multicolumn{1}{c}{(2)}  &    &\multicolumn{1}{c}{(3)}   &   \multicolumn{1}{c}{(4)}    &  &\multicolumn{1}{c}{(5)}      &\multicolumn{1}{c}{(6)}      \\

\midrule

&&&&&&&\\
\textbf{Tax effect on prices }            &                          0.038\sym{***}&               0.038\sym{***}&   &                        0.041\sym{***}&               0.041\sym{***} & &  0.038\sym{***}& 0.038\sym{***} \\
                    &                  (0.004)         &             (0.004)       &      &             (0.005)         &             (0.005)     & &    (0.005)         &  (0.005)  \\
&&&&&&&\\
\midrule
Observations        &                    1,936,322         &             1,936,322       &         &             1,290,843         &             1,290,843   & &   1,276,400         &             1,276,400          \\
\(R^{2}\)           &                          0.759         &               0.811      &         &               0.754         &               0.809        & &     0.699         &               0.747 \\


\midrule

Constant            &                               Yes         &                 Yes       &  &Yes         &                 Yes       &  &Yes         &                 Yes    \\

Time FE             &                        Yes         &                 Yes    &     &                           Yes         &                 Yes       &  &Yes         &                 Yes    \\

Agency FE           &                             Yes         &                  No       &  &                            Yes         &                  No      &  &Yes         &                 No    \\

League FE           &                              Yes         &                  No     &    &                             Yes         &                  No       &  &Yes         &                 No   \\

League-agency FE    &                            No         &                 Yes      &   &                      No         &                 Yes     &  &No         &                 Yes      \\
\hline \hline
\multicolumn{8}{l}{\footnotesize Standard errors in parentheses. \sym{*} \(p<0.05\), \sym{**} \(p<0.01\), \sym{***} \(p<0.001\)}\\
\end{tabular}
}
\end{table}



==> Figures_tex/Onshore_offshore.tex <==
	\begin{figure}[!ht]
		\caption{Onshore vs. Offshore gross online betting revenues in Germany (in Mio. Euro)}
		%	\label{fig:bettingrevenues_ger}

		\centering	
	
		\includegraphics[width=15cm]{digtax/Figures/Onshore_Offshore_revenues.png}
		\begin{minipage}{14.8cm}  \footnotesize  \emph{Notes:} 
			This  figure  illustrates the annual total gross online betting revenues between 2008 and 2020 in Germany (in mio Euro), disaggregated in onshore and offshore betting revenues. The bars illustrate the share of onshore betting revenues. Onshore revenues refer to all sports betting activities for which taxes were paid in Germany. For 2012, the onshore revenues refer to all revenues by agencies that paid sports betting taxes in 2012. Offshore revenues include all sports betting revenues by agencies that target the German market, but do not pay the sports betting tax in Germany. Gross betting revenues are equal to the total wagered amount (including bonuses) minus all winnings by bettors, disaggregated by onshore and offshore agencies. Data was provided by H2 Gambling Capital (July 2021) and is primarily based on official data by official gambling regulatory bodies, governments and tax authorities.\footnote{H2 further uses information from monopoly data where available for land-based and onshore interactive activity and information derived from major operators and suppliers active in each market, including their publicly available reports. To determine whether a agency target a particular market, H2 undertakes a biannual audit of all operators, examining whether agencies proactively targeting domestic players, accepting domestic players, or (not) prohibiting domestic players from betting. In allocating activity across markets, H2 then take into account any actual market/regional information they hold/receive/is disseminated by companies, the experience we have developed (they have undertaken the quarterly supply assessment for the past 12 years as well as one-off deeper dive assessments into markets), feedback from users (we currently have well over 1,000 users with access to our subscriber area many of whom work on the ground with interactive operators / suppliers). Furthermore, they also consider any restrictions that are in place, any onshore supply and several generic measures ranging from GDP to broadband / smartphone penetration to sense check the size of each market. (Email by H2). } The data does only include revenues of operators that are licensed in at least one jurisdiction. Completely unlicensed activities are not included.
		\end{minipage}
	\end{figure}


==> Figures_tex/Policies_example.tex <==
    \begin{figure}[!ht]
     	\caption{Example of different "shrouding" policies}
     	 %\label{fig:policies}

        \begin{minipage}[b]{0.31\linewidth}
            \centering
            \caption*{i) No further deductions}
            \includegraphics[width=\textwidth]{digtax/Tipico_Taxdis_pras.png}
            \label{fig:a}
        \end{minipage}
        \hspace{0.2cm}
        \begin{minipage}[b]{0.31\linewidth}
            \centering
            \caption*{ii) Deduction of winnings}
            \includegraphics[width=\textwidth]{digtax/Bwin_Taxdis_pras.png}
            \label{fig:b}
        \end{minipage}
            \hspace{0.2cm}
        \begin{minipage}[b]{0.31\linewidth}
            \centering
            \caption*{iii) Deduction of wager}
            \includegraphics[width=\textwidth]{digtax/Betathome_Taxdis_pras.png}
            \label{fig:c}
        \end{minipage}
        \begin{minipage}{13.8cm}  \footnotesize  \emph{Notes:} 
			This  figure  presents an examples of the presentation of different betting slips (browser version) after you choose one of the outcomes: a draw on the game between Chelsea FC and Manchester City in our example. The gross odds on the top are presented, excluding the tax, for all three panels. All of the betting slips show the potential net payouts on the bottom. The size of the net payouts depend on different "shrouding" policies: i) No (additional) deduction of taxes, i.e., effective tax inclusive odds are equal to tax exclusive odds; ii) deduction of 5\% of the winning, i.e., effective tax inclusive odds are equal to 95\% of the tax-exclusive odds; iii) deduction of 5\% of the wager, i.e., the effective tax-inclusive odds are equal to: $1/1.05$ of the tax-exclusive odds. Note that example iii) already applies the new tax rate of 5.3\%, which was introduced in Juli 2021.  Source: i) Tipico.com; ii) bwin.com; iii) Bet365.com  - September 2021.  
		\end{minipage}
    \end{figure}


==> Figures_tex/Tax_revenue.tex <==
		\begin{figure}[!ht]
		\caption{German Sports Betting Tax Revenue 2012-2020 in Mio. Euro}
		\centering	
	
		\includegraphics[width=15cm]{digtax/Figures/Tax_revenues_charts.png}
		\begin{minipage}{14.8cm}  \footnotesize  \emph{Notes:} 
			This  figure  illustrates the aggregated annual tax revenue generated by the German sports betting tax between 2012 and 2020. The tax revenue in 2012 only covers a period of 6 months, as the tax was introduced at 1 July 2012. Source: German Federal Ministry of Finance.  
		\end{minipage}
		  \label{fig:tax_revenues}
	\end{figure}


==> Figures_tex/Total_stakes.tex <==
		\begin{figure}[!ht]
		\caption{Total wagered stakes and gross win margins in Germany}
		\centering	
	
		\includegraphics[width=15cm]{digtax/Figures/Total Stakes and Gross win margins.png}
		\begin{minipage}{14.8cm}  \footnotesize  \emph{Notes:} 
        The solid line illustrates the total wagered amount in Germany between 2012 and 2020, based on the official tax data. The grey bars presents the implied gross win margins of the betting agencies, which are equal to the gross betting revenues (provided by H2) divided by the total wagered amount. 
		\end{minipage}
		  \label{fig:grosswinmargins}
	\end{figure}
	

==> Figures_tex/all_figures.tex <==

%\input{digtax/Figures_tex/total_revenue}

%\input{digtax/Figures_tex/Onshore_offshore}

%\input{digtax/Figures_tex/Tax_revenue}

%\input{digtax/Figures_tex/Example_odds}

%\input{digtax/Figures_tex/Policies_example}

%\input{digtax/Figures_tex/Avg_prices_all.tex}

%\input{digtax/Figures_tex/TWFE_all}

%\input{digtax/Figures_tex/TWFE_het}


\newpage

%\input{Figures_tex/Total_stakes}

==> Figures_tex/hist_policies.tex <==
\begin{figure}[!ht]

    \centering
      \caption{Effect of tax on consumer betting prices over time - agencies where data is availbale for all year}
          \begin{subfigure}[t]{0.48\textwidth}
        \centering
        \caption{ All sports }
        \includegraphics[width=\linewidth]{digtax/Figures/coef_allsports_all_agencies_tipico.png} 
         \label{fig:timing1}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.48\textwidth}
        \centering
         \caption{ All sports - excluding cross leagues }
        \includegraphics[width=\linewidth]{digtax/Figures/coef_allsports_all_agencies_tipico_hard.png} 
        \label{fig:timing2}
    \end{subfigure}
          \vspace{0.5cm}

     \begin{subfigure}[t]{0.48\textwidth}
        \centering
        \caption{ Only soccer games}
        \includegraphics[width=\linewidth]{digtax/Figures/coef_soccer_compl_agencies_tipico.png} 
        \label{fig:timing1}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.48\textwidth}
        \centering
        \caption{ Only soccer games - excluding cross leagues}
        \includegraphics[width=\linewidth]{digtax/Figures/coef_soccer_compl_agencies_tipico_hard.png} 
         \label{fig:timing2}
    \end{subfigure}
      \vspace{0.5cm}
  
    \begin{subfigure}[t]{0.48\textwidth}
        \centering
        \caption{ All sports }
        \includegraphics[width=\linewidth]{digtax/Figures/coef_allsports_compl_agencies_tipico.png} 
         \label{fig:timing1}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.48\textwidth}
        \centering
         \caption{ All sports - excluding cross leagues }
        \includegraphics[width=\linewidth]{digtax/Figures/coef_allsports_compl_agencies_tipico_hard.png} 
        \label{fig:timing2}
    \end{subfigure}


     		\begin{minipage}{16cm}  \footnotesize  \emph{Notes:} 
This figures shows the estimated effects and respective 95-\% confidence intervals of the German sports-betting tax on consumers' betting prices over time. Only agencies for which odds data in all years is available are considered, N=30 (Treatment=9/Control=21). Panel (a) and (b) consider all sports included in the data set, while Panel (c) and (d) only consider soccer events. Panel (b) and (d) excludes German leagues for the control group and Non-German leagues for the treatment group. The vertical dashed line illustrates the introduction of the tax reform. The horizontal dotted line signifies a full-pass through of the tax on consumers.
		\end{minipage} 
		\label{fig:coef robust}
  
\end{figure} 

==> Figures_tex/total_revenue.tex <==


		\begin{figure}[!ht]
		\caption{Total online gross betting revenues in different countries (in million Euro)}
		\centering	
	
		\includegraphics[width=15cm]{digtax/Figures/Betting_revenues_countries.png}
		\begin{minipage}{14.8cm}  \footnotesize  \emph{Notes:} 
			This  figure  illustrates the annual total online gross betting revenues between 2008 and 2020 in Germany, Italy and France. Gross betting revenues are equal to the total wagered amount (including bonuses) minus all winnings by bettors. Revenues include both onshore (i.e. regulated/taxed activity) and offshore (i.e. revenue of operators targeting the market without holding a local license) revenues.  Source: H2 Gambling Capital – July 2021.  
		\end{minipage}
		%  \label{fig:bettingrevenues_countries}
	\end{figure}

==> Summary.tex <==
\begin{table}[!htbp]\centering
%\tiny
\caption{Summary statistics - Betting prices}
\label{tab:sum_price}
\scalebox{0.87}{
    \begin{tabular}{l|ccc}
    \multicolumn{1}{c|}{League - Sport} & Mean  & Std.Dev. & Observations \\ \hline
     \textbf{All agencies:}     &       &       &  \\[0.5em]
    All events & 0.0706 & 0.0317 & 3,289,135 \\ 
    Soccer events     &  0.0734     &   0.0315    & 2,067,137  \\ \hline
\textbf{German agencies by shrouding } &       &       &  \\
\textbf{policy (pre-reform):} &       &       &  \\[0.5em]    
No "shrouding" (i) & 0.0737 & 0.0199 & 24,351 \\
Deduction from winnings (ii)  & 0.0726 &  0.0225 & 143,842 \\
Deduction from wager (iii) & 0.0745 & 0.0207 & 47,068 \\

    \hline \hline
    \end{tabular}%
}
\end{table}



==> Tables/DiffinDiff_het.tex <==
\begin{table}[htbp]\centering
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\caption{Soccer - all agencies}
\scalebox{0.9}{
\begin{tabular}{l*{9}{c}}
\hline\hline

                 &\multicolumn{4}{c}{All Leagues}     & &\multicolumn{4}{c}{Excl. "cross" leagues}     \\    \cmidrule{2-5} \cmidrule{7-10}
                                  &\multicolumn{2}{c}{Subsamples}     & \multicolumn{2}{c}{Interactions}  &\multicolumn{4}{c}{Excl. "cross" leagues}     \\ 
                    &\multicolumn{1}{c}{(1)}      &\multicolumn{1}{c}{(2)}      &\multicolumn{1}{c}{(3)}      &\multicolumn{1}{c}{(4)}      & &\multicolumn{1}{c}{(5)}      &\multicolumn{1}{c}{(6)}      &\multicolumn{1}{c}{(7)}      &\multicolumn{1}{c}{(8)}      \\

\midrule
Tax effect on prices           &               0.008\sym{***}&               0.041\sym{***}&               0.046\sym{***}&               0.046\sym{***}&    &           0.008\sym{**} &               0.045\sym{***}&               0.050\sym{***}&               0.050\sym{***}\\
                    &             (0.002)         &             (0.003)         &             (0.003)         &             (0.003)         &  &           (0.002)         &             (0.003)         &             (0.003)         &             (0.003)         \\
[1em]
Treat x no "shroud"          &                             &                             &              -0.041\sym{***}&              -0.041\sym{***}&                             &                             &  &            -0.043\sym{***}&              -0.043\sym{***}\\
                           &                      &                             &             (0.002)         &             (0.002)         &     &                        &                             &             (0.002)         &             (0.002)         \\
[1em]
Constant            &               0.085\sym{***}&               0.084\sym{***}&               0.084\sym{***}&               0.084\sym{***}&   &            0.091\sym{***}&               0.091\sym{***}&               0.091\sym{***}&               0.091\sym{***}\\
                    &             (0.003)         &             (0.003)         &             (0.003)         &             (0.003)         &   &          (0.003)         &             (0.003)         &             (0.003)         &             (0.003)         \\
\midrule
Time FE             &                 Yes         &                 Yes         &                 Yes         &                 Yes         &  &               Yes         &                 Yes         &                 Yes         &                 Yes         \\
Agency FE           &                 Yes         &                 Yes         &                 Yes         &                 Yes         &    &             Yes         &                 Yes         &                 Yes         &                 Yes         \\
League FE           &                 Yes         &                 Yes         &                 Yes         &                 Yes         &   &              Yes         &                 Yes         &                 Yes         &                 Yes         \\
\midrule
Observations        &             1,587,090         &             1,881,406         &             1,936,322         &             1,936,322         &     &        1211548         &             1277394         &             1290843         &             1290843         \\
\(R^{2}\)           &               0.728         &               0.767         &               0.779         &               0.779         &   &            0.737         &               0.757         &               0.761         &               0.761         \\
\hline\hline
\multicolumn{9}{l}{\footnotesize Standard errors in parentheses}\\
\multicolumn{9}{l}{\footnotesize \sym{*} \(p<0.05\), \sym{**} \(p<0.01\), \sym{***} \(p<0.001\)}\\
\end{tabular}
}
\end{table}


==> Tables/Tables.tex <==
\input{Tables/DiffinDiff_het_pol}
